The Fundamental Memory Ceiling of Noisy Quantum Reservoirs

Fresh qubits, not size, set how long a noisy quantum system can remember. With $k$ input qubits reinitialized per time step, the longest memory any reservoir can attain under depolarizing noise is $\exp[\Theta(k)]$ time steps, whatever its size, dynamics, and input encoding. A universal upper bound and an explicit reservoir that attains the exponential scaling establish this optimal resource law. The bound depends on the dynamics only through the entropy that fresh qubits remove per time step, so it holds for any Markovian noisy dynamics without feedback, including measurement-free error correction.

==> figure_sources/tikzstyle.tex <==
% Shared TikZ style for the schematics. Same typeface, size (8 pt) and palette as figstyle.py:
% blue = memory / reservoir dynamics, red = noise and the limit, purple = input, greys = neutral.
\usepackage[T1]{fontenc}
\ifdefined\pdfgentounicode\input{glyphtounicode}\pdfgentounicode=1\fi
\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}
\usepackage{amsmath,amssymb,bm}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,calc,decorations.pathreplacing,patterns.meta,shapes.geometric,shadows}
\definecolor{cInk}{HTML}{1A1A1A}
\definecolor{cBlue}{HTML}{3C7FE0}
\definecolor{cBlueDark}{HTML}{1D4C9C}
\definecolor{cBlueLight}{HTML}{8DB8F0}
\definecolor{cBlueFill}{HTML}{DDE9F9}
\definecolor{cRed}{HTML}{EF4B3B}
\definecolor{cRedDark}{HTML}{B8301F}
\definecolor{cRedFill}{HTML}{FCE3DE}
\definecolor{cPurple}{HTML}{9B4FE0}
\definecolor{cPurpleDark}{HTML}{6B2CAB}
\definecolor{cPurpleFill}{HTML}{EFE2FB}
\definecolor{cGreyDark}{HTML}{4A4A4A}
\definecolor{cGrey}{HTML}{8C8C8C}
\definecolor{cGreyLight}{HTML}{B4B4B4}
\definecolor{cGreyFill}{HTML}{EDEDED}
\definecolor{cShadow}{HTML}{B5B5B5}
\tikzset{
  every node/.style={font=\fontsize{8}{9.6}\selectfont},
  lbl/.style={font=\fontsize{8}{9.6}\selectfont},
  ttl/.style={font=\fontsize{8}{9.6}\selectfont,anchor=base west,inner sep=0pt},
  ttlr/.style={font=\fontsize{8}{9.6}\selectfont,anchor=base east,inner sep=0pt},
  wire/.style={line width=0.65pt,cInk},
  ublk/.style={draw=cInk,line width=0.6pt,fill=cBlue,rounded corners=1.6pt},
  iblk/.style={draw=cInk,line width=0.6pt,rounded corners=1.6pt,preaction={fill=cPurple},
    pattern={Lines[angle=55,distance=2.2pt,line width=0.85pt]},pattern color=white},
  nbox/.style={draw=cInk,line width=0.55pt,fill=cRed,rounded corners=1.1pt},
  feat/.style={draw=cInk,line width=0.6pt,fill=white,rounded corners=2pt,inner sep=1.6pt,
    minimum width=0.98cm,minimum height=0.44cm},
  legbox/.style={draw=cInk,line width=0.8pt,fill=white,rounded corners=2.4pt,
    drop shadow={shadow xshift=1.2pt,shadow yshift=-1.2pt,fill=cShadow,opacity=1}},
  arr/.style={line width=0.65pt,-{Stealth[length=3.6pt,width=3.2pt]}},
  brc/.style={decorate,decoration={brace,amplitude=2.6pt},line width=0.55pt},
}
\newcommand{\Discard}[3][cInk]{%
  \draw[line width=0.75pt,#1] (#2,{#3-0.1}) -- (#2,{#3+0.1});
  \draw[line width=0.75pt,#1] ({#2+0.05},{#3-0.064}) -- ({#2+0.05},{#3+0.064});
  \draw[line width=0.75pt,#1] ({#2+0.1},{#3-0.03}) -- ({#2+0.1},{#3+0.03});}
\providecommand{\ket}[1]{|#1\rangle}
\providecommand{\nrm}[2]{\lvert #1\rvert_{#2}}

